Scale-out Systolic Arrays

Multi-pod systolic arrays are emerging as the architecture of choice in DNN inference accelerators. Despite their potential, designing multi-pod systolic arrays to maximize effective throughput/Watt (i.e., throughput/Watt adjusted when accounting for array utilization) poses a unique set of challenges. In this work, we study three key pillars in multi-pod systolic array designs, namely array granularity, interconnect, and tiling. We identify optimal array granularity across workloads and show that state-of-the-art commercial accelerators use suboptimal array sizes for single-tenancy workloads. We, then evaluate the bandwidth/latency trade-offs in interconnects and show that Butterfly networks offer a scalable topology for accelerators with a large number of pods. Finally, we introduce a novel data tiling scheme with custom partition size to maximize utilization in optimally sized pods. We propose Scale-out Systolic Arrays, a multi-pod inference accelerator for both single- and multi-tenancy based on these three pillars. We show that SOSA exhibits scaling of up to 600 TeraOps/s in effective throughput for state-of-the-art DNN inference workloads, and outperforms state-of-the-art multi-pod accelerators by a factor of 1.5x.

==> tex/algo.tex <==

\begin{algorithm}[!h]
%  \KwData{this text}
%  \KwResult{how to write algorithm with \LaTeX2e }

\KwIn{$g$: Tile operation}

 $l \gets$ find layer's beginning round
 
 \While{$g$ is not scheduled}{
    $S_{idle} \gets$ find idle systolic pods in round $l$ \;
  
    $X_{idle} \gets$ find available $X$ banks in round $l$ \;
  
    $W_{idle} \gets$ find available $W$ banks in round $l$ \;
    
    $P_{idle} \gets$ find available $P$ banks in round $l$ \;
    
    \ForEach{$s$ in $S_{idle}$}{
        \ForEach{$x$ in $X_{idle}$}{
            \If{$x \rightarrow s$ is \textbf{not} free }{continue\;}
  
            \ForEach{$w$ in $W_{idle}$}{
                \If{$w \rightarrow s$ is \textbf{not} free }{continue\;}
                
                \ForEach{$p$ in $P_{idle}$}{
                \eIf{$s \rightarrow p$ is \textbf{not} free }{continue\;}{
                    assign $g$ to $s$ in round $l$\;
                    
                    assign tiles to bank $x$, $w$, and $p$\;
                    
                    return \;
                }
                }
                
            }
        }  
    }
    
    $r \gets r+1$\;
 
  
 }
 \caption{The proposed mapping and scheduling algorithm. $a \rightarrow b$ represents the interconnect path from $a$ to $b$}
 \label{algo:scheduler}
\end{algorithm}



==> tex/ict_table.tex <==
\begin{tabular}{r|c|c|c|c|c}
% Network type & %
% Appeared in & %
% \begin{tabular}[c]{@{}c@{}}Bisection BW\\ (number of links)\end{tabular} & %
% \begin{tabular}[c]{@{}c@{}}Combinatorial power \\w/ multicast \end{tabular} & %
% \begin{tabular}[c]{@{}c@{}}Latency \\ (cycles)\end{tabular} & %
% \begin{tabular}[c]{@{}c@{}}Hardware cost\\ (number of switches)\end{tabular} \\\hline

Type &
Ref. &
\multrowC{Bisection\\BW} &
\multrowC{Combinatorial\\Power with\\Multicasts} &
\multrowC{Latency\\ \lbrack cycles\rbrack} &
Cost\\\hline

2D Mesh & %
\multrowC{\cite{Chen17}\cite{Chen14}\\\cite{gao19}\cite{shao19}} & %
$\sqrt{N}$ & %
Low & %
$\sqrt{N}$ & $N$ \\\hline

H-tree & %
\cite{Stevens19} & %
1 & %
Low & %
$\log{N}$ & %
$N$\\ \hline

\multrowR{H-tree\\(scaled-up)} & %
\cite{kung2019} & %
N & %
Full & %
$\log{N}$ & %
$N^2$\\ \hline

Crossbar & %
\cite{Zhu20} & %
$N$ & %
Full & 1 & $N^2$ \\\hline

\begin{comment}
Benes & %
\cite{Qin20} & %
$N$ & %
High & %
$2\log N$ & %
$N\log N$ \\\hline
\end{comment}

\multrowR{Benes w/\\ copy network} & %
\cite{liew2010} & %
$N$ & %
Full & %
$4\log N$ & %
$2N\log N$ \\\hline

Butterfly & %
  & %
$N$ & %
Low & %
$\log{N}$ & %
$(N/2) \log N$ \\\hline

\textbf{Butterfly-k} & %
This work & %
$kN$ & %
High & %
$\log{kN}$ & %
$(kN/2) \log N$

\end{tabular}

